On the use of Large Language Models in Model-Driven Engineering

Model-Driven Engineering (MDE) has seen significant advancements with the integration of Machine Learning (ML) and Deep Learning (DL) techniques. Building upon the groundwork of previous investigations, our study provides a concise overview of current Language Large Models (LLMs) applications in MDE, emphasizing their role in automating tasks like model repository classification and developing advanced recommender systems. The paper also outlines the technical considerations for seamlessly integrating LLMs in MDE, offering a practical guide for researchers and practitioners. Looking forward, the paper proposes a focused research agenda for the future interplay of LLMs and MDE, identifying key challenges and opportunities. This concise roadmap envisions the deployment of LLM techniques to enhance the management, exploration, and evolution of modeling ecosystems. By offering a compact exploration of LLMs in MDE, this paper contributes to the ongoing evolution of MDE practices, providing a forward-looking perspective on the transformative role of Language Large Models in software engineering and model-driven practices.

==> agenda_src/Claudio_notes.tex <==
\section{Claudio Notes}



\subsection{Evaluating the hallucination in modeling}
The LLMs hallucination phenomenon \cite{ji_survey_2023} is a well-know issue in SE that could lead to unwanted results. In the MDE context, we can study the impact of this issue by consider human-in-the-loop, \ie modelers. Process mining techniques \cite{dehghanitowards} \CDS{Juri JJODEL can be inserted here} have been proposed to collect modelers' behavior during the specification of the model under construction. We can use the real data to measuring the hallucination using real data.  



\subsection{Building an extensive model ontology for feeding LLMs}
Ontologies in SE have been proposes to enhance automated approaches \cite{izadi_semantically-enhanced_2023}. In this respect, LLMs may leverage on domain knowledge to improve the generated recommendations. Such a knowledge base can be used to perform retrieval augmented generation (RAG) specifically conceived for modeling. 




==> agenda_src/Juri_notes.tex <==

\section{Juri Notes}



\subsection{Evaluation LLM performances}
\begin{itemize}
	\item Evaluation methodologies:
	\begin{itemize}
		\item Holdout Validation (Split Validation): This involves splitting the dataset into two parts: a training set and a testing set. A common split is 80/20, where 80\% of the data is used for training the model and 20\% is used for testing its performance. This is the most used one;
		\item K-Fold Cross-Validation: The dataset is divided into 'k' subsets. The model is trained on 'k-1' subsets and tested on the remaining subset. This process is repeated 'k' times, with each subset serving as the test set once. The results are then averaged to estimate the model's performance. This is not always doable with LLM because of the cost of fine tuning the model;
		\item Leave-one-out cross-validation: A form of cross-validation where each instance in the dataset is used once as a single observation in the test set. This method is computationally expensive but can be beneficial for small datasets. This method is very rare because of the number of fine tuning models steps;
		\item User study or user evaluation: Involves real users interacting with the model and providing feedback on its performance. This is particularly important for applications where human-like interaction or understanding is crucial;
		\item Random subsampling: Similar to K-fold cross-validation, but the splits are done randomly. This is repeated several times, and the average performance is considered.
	\end{itemize}
	\item Evaluation metrics
	\begin{itemize}
		\item Standard metrics, \ie Accuracy, precision, recall and F1 Score: Measuring the accuracy of responses, especially in tasks like classification or question-answering, to determine how often the model provides the correct answer.
		\item BLEU Score: Commonly used in machine translation, this metric evaluates the quality of text that has been machine-translated from one language to another.
		\item ROUGE Score: Evaluating the quality of summary texts generated by the model, focusing on the overlap between the generated text and a set of reference summaries.
  		\item METEOR~\cite{meteor}
	\end{itemize}
\end{itemize}
